On Implementing Real-time Specification Patterns Using Observers

English language requirements are often used to specify the behavior of complex cyber-physical systems. The process of transforming these requirements to a formal specification language is often challenging, especially if the specification language does not contain constructs analogous to those used in the original requirements. For example, requirements often contain real-time constraints, but many specification languages for model checkers have discrete time semantics. Work in specification patterns helps to bridge these gaps, allowing straightforward expression of common requirements patterns in formal languages. In this work we demonstrate how we support real-time specification patterns in the Assume Guarantee Reasoning Environment (AGREE) using observers. We demonstrate that there are subtle challenges, not mentioned in previous literature, to express real-time patterns accurately using observers. We then demonstrate that these patterns are sufficient to model real-time requirements for a real-world avionics system.

==> agree-overview.tex <==
\section{Compositional Verification with AGREE}\label{sec:comp-v}

In this section we briefly describe the rules that AGREE uses to create compositional proofs. A more complete description is in~\cite{CoferNFM2012} and a proof of correctness of these rules is provided in~\cite{AgreeUsersGuide,CoferNFM2012}.

AGREE is a language and a tool for compositional verification of AADL models.  The behavior of a model is described by \textit{contracts} specified on each component.  A contract contains a set of \textit{assumptions} about the component's inputs and a set of \textit{guarantees} about the component's outputs.  The assumptions and guarantees may also contain predicates that reason about how the state of a component evolves over time. The state transitions of each component in the model occur synchronously with every other component (i.e., each component runs on the same clock).  The guarantees of a component must be true provided that the component's assumptions have always been true.  The goal of the analysis is to prove that a component's contract is entailed by the contracts of its subcomponents.

Formally, let a system $S : (A,G,C)$ consist of a set of assumptions $A$, guarantees $G$, and subcomponents $C$. We use the notation $S_g$ to represent the conjunction of all guarantees of $S$ and $S_a$ to represent the conjunction of all assumptions of $S$. Each subcomponent $c \in C$ is itself a system with assumptions, guarantees, and subcomponents. The goal of our analysis is to prove that the system's guarantees hold as long as its assumptions have always held.  This is accomplished by proving that Formula~\ref{fml:obligation} is an invariant.

\begin{center}
\begin{equation}\label{fml:obligation}
\mathbf{H}(S_a) \rightarrow S_g
\end{equation}
\end{center}

The predicate $\mathbf{H}$ is true if its argument has held \textit{historically} (i.e., the expression has been true at every time step up until and including now). In order to prove that Formula~\ref{fml:obligation} is invariant, we prove that the assumptions of all the subcomponents of system $S$ hold under the assumptions of $S$. This invariant is shown in Formula~\ref{fml:strong-assump}.

\begin{center}
\begin{equation}\label{fml:strong-assump}
\bigwedge_{c\in C} \Big[ \mathbf{H}(S_a) \rightarrow c_a \Big]
\end{equation}
\end{center}

This formula is actually stronger than what we need to prove.  It may be the case that the assumptions of certain subcomponents are satisfied by the guarantees of other subcomponents (and possibly the guarantees of the component itself at previous instances in time).  This weaker invariant is shown in Formula~\ref{fml:weak-assump}.

\begin{center}
\begin{equation}\label{fml:weak-assump}
 \bigwedge_{c\in C} \Big[ \Big( \mathbf{H}(S_a) \wedge \bigwedge_{w \in C} \mathbf{Z}(\mathbf{H}(w_g))\wedge\bigwedge_{v \in C, c \neq v} \mathbf{H}(v_g) \Big) \rightarrow c_a \Big]
\end{equation}
\end{center}

The predicate $\mathbf{Z}$ is true in the first step of a trace and thereafter is true iff its argument was true in the previous time step. 

However, this formula may not be sound when the connections between components form cycles.  One could imagine a scenario where the assumptions of each of two components are true precisely because of the guarantees of the other component (i.e., $w_g \rightarrow v_a $ and $v_g \rightarrow w_a$ for $w,v \in C$ and $w \neq v$). Suppose components $w$ and $v$ both assume that their inputs are positive, and they guarantee that their outputs are positive.  If the output of $w$ is connected to the input of $v$, and $v$'s output is connected to $w$, the state of the system is improperly defined.  To avoid this problem, AGREE  creates a total ordering of a system's subcomponents.  It uses this ordering to determine which subcomponent guarantees are used to prove the assumptions of other subcomponents.  This slight modification of Formula~\ref{fml:weak-assump} is shown in Formula~\ref{fml:correct-assump}.

\begin{center}
\begin{equation}\label{fml:correct-assump}
\bigwedge_{c\in C} \Big[ \Big( \mathbf{H}(S_a) \wedge \bigwedge_{w \in C}\mathbf{Z}(\mathbf{H}(w_g))\wedge\bigwedge_{v \in C, v < c} \mathbf{H}(v_g) \Big) \rightarrow c_a \Big]
\end{equation}
\end{center}

If Formula~\ref{fml:correct-assump} is invariant then Formula~\ref{fml:obligation} is proven to be invariant by showing that the system assumptions and subcomponent guarantees satisfy the system guarantees.  Formally, if Formula~\ref{fml:correct-assump} is invariant, then Formula~\ref{fml:guar-check} implies Formula~\ref{fml:obligation}.

\begin{center}
\begin{equation}\label{fml:guar-check}
 \mathbf{H}(S_a) \wedge \bigwedge_{c \in C} \mathbf{H}(c_g) \rightarrow S_g
\end{equation}
\end{center}

AGREE uses a syntax similar to Lustre to express a contract's assumptions and guarantees~\cite{lustre}. AGREE translates an AADL model annotated with AGREE annexes into Lustre corresponding to Formulas~\ref{fml:correct-assump} and~\ref{fml:guar-check} and then queries a user selected model checker. AGREE then translates the results from the model checker back into OSATE so they can be interpreted by the user. For this project we have used both the Kind 2.0 and JKind model checkers~\cite{kind2,Jkind}.

In Section~\ref{sec:reqs} we describe some examples of guarantees that were written in AGREE to model some of the requirements in the QFCS architecture.  However, the examples are presented here in a simple first order logic syntax to make them more concise and readable.




